Automatic Generators for a Family of Matrix Multiplication Routines with Apache TVM

We explore the utilization of the Apache TVM open source framework to automatically generate a family of algorithms that follow the approach taken by popular linear algebra libraries, such as GotoBLAS2, BLIS and OpenBLAS, in order to obtain high-performance blocked formulations of the general matrix multiplication (GEMM). % In addition, we fully automatize the generation process, by also leveraging the Apache TVM framework to derive a complete variety of the processor-specific micro-kernels for GEMM. This is in contrast with the convention in high performance libraries, which hand-encode a single micro-kernel per architecture using Assembly code. % In global, the combination of our TVM-generated blocked algorithms and micro-kernels for GEMM 1)~improves portability, maintainability and, globally, streamlines the software life cycle; 2)~provides high flexibility to easily tailor and optimize the solution to different data types, processor architectures, and matrix operand shapes, yielding performance on a par (or even superior for specific matrix shapes) with that of hand-tuned libraries; and 3)~features a small memory footprint.

==> biography/biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biography/foto_guille.jpg}}]
{\textbf{Guillermo Alaejos L\'opez}} received his bachelor in Computer Science from Universitat Jaume I in 2020, he is a master student in Cloud Computing and High Performance Computing at Universitat Polit\`ecnica de Val\`encia (expected graduation April 2022). His research interests covers the code auto-generation as well as high-performance applications.%He is going to do his Ph.D. degree in Universitat Polit\'ecnica de Val\'encia.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biography/adrian.jpeg}}]
{\textbf{Adri\'an Castell\'o}} received his bachelor, M.Sc. and Ph.D. degrees in Computer Science from Universitat Jaume I in 2011, 2013 and 2018, respectively. He is a Postdoc researcher at the Universitat Polit\`ecnica de Val\`encia and his research interests include high-performance computing, code auto-generation, deep neural networks, and programming models.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biography/PedroAlonsoPicture.jpg}}]
{\textbf{Pedro Alonso-Jord\'a}} received the bachelor (1994) and Ph.D. (2003) degrees in Computer Science from Universitat Polit\`ecnica de Val\`encia. 
He has been developing his academic activity since 1996 at this university, where currently 
is Full Professor. 
His research field is in High Performance Computing being the main research areas 
heterogeneous parallel computing and energy aware computing. He currently is director of the Master's degree in Cloud and High-Performance Computing.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biography/foto_enrique.jpg}}]
{\textbf{Enrique S. Quintana-Ort\'i}} received bachelor and Ph.D. degrees in Computer Science from Universitat Polit\`ecnica de Val\`encia (UPV), Spain, in 1992 and 1996, respectively. After more than 20 years at Universitat Jaume~I, he is currently Professor in Computer Architecture at UPV. His current research interests include parallel programming, linear algebra, energy consumption, transprecision computing and deep learning as well as advanced architectures and hardware accelerators.
\end{IEEEbiography}

\begin{IEEEbiography}%
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biography/fran.jpeg}}]
{Francisco D. Igual}
    obtained a bachelor degree in Computer Engineering from University Jaume I de Castellón (Spain) in 2006, and a Ph.D. degree in Computer Science from the same University in 2011. In 2011, he moved as a postdoctoral researcher to The University of Texas at Austin, and in 2012 he joined the Universidad Complutense de Madrid where he is currently Associate Professor.
His research interests include high-performance and energy-aware computing, dense linear algebra library development and optimization, and runtime task scheduling on massively heterogeneous architectures. 
%He has co-authored more than 50 papers in journals and conferences in the aforementioned fields.
\end{IEEEbiography}


%

==> plots/Results/ARM/Algorithm_ARM_006-lines.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(682,1263){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(682,1782){\makebox(0,0)[r]{\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(682,2302){\makebox(0,0)[r]{\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(682,2821){\makebox(0,0)[r]{\strut{}$15$}}%
      \csname LTb\endcsname%%
      \put(682,3340){\makebox(0,0)[r]{\strut{}$20$}}%
      \csname LTb\endcsname%%
      \put(682,3860){\makebox(0,0)[r]{\strut{}$25$}}%
      \csname LTb\endcsname%%
      \put(682,4379){\makebox(0,0)[r]{\strut{}$30$}}%
      \put(906,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times4$}}}%
      \put(998,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times8$}}}%
      \put(1090,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times12$}}}%
      \put(1183,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times16$}}}%
      \put(1275,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times20$}}}%
      \put(1367,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times24$}}}%
      \put(1459,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times28$}}}%
      \put(1551,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times32$}}}%
      \put(1643,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times4$}}}%
      \put(1735,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times8$}}}%
      \put(1828,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times12$}}}%
      \put(1920,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times16$}}}%
      \put(2012,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times20$}}}%
      \put(2104,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times24$}}}%
      \put(2196,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times28$}}}%
      \put(2288,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times32$}}}%
      \put(2380,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times4$}}}%
      \put(2472,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times8$}}}%
      \put(2565,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times12$}}}%
      \put(2657,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times16$}}}%
      \put(2749,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times20$}}}%
      \put(2841,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times24$}}}%
      \put(2933,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times28$}}}%
      \put(3025,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times32$}}}%
      \put(3117,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times4$}}}%
      \put(3210,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times8$}}}%
      \put(3302,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times12$}}}%
      \put(3394,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times16$}}}%
      \put(3486,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times20$}}}%
      \put(3578,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times24$}}}%
      \put(3670,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times28$}}}%
      \put(3762,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times32$}}}%
      \put(3855,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times4$}}}%
      \put(3947,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times8$}}}%
      \put(4039,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times12$}}}%
      \put(4131,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times16$}}}%
      \put(4223,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times20$}}}%
      \put(4315,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times24$}}}%
      \put(4407,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times28$}}}%
      \put(4500,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times32$}}}%
      \put(4592,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times4$}}}%
      \put(4684,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times8$}}}%
      \put(4776,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times12$}}}%
      \put(4868,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times16$}}}%
      \put(4960,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times20$}}}%
      \put(5052,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times24$}}}%
      \put(5145,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times28$}}}%
      \put(5237,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times32$}}}%
      \put(5329,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times4$}}}%
      \put(5421,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times8$}}}%
      \put(5513,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times12$}}}%
      \put(5605,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times16$}}}%
      \put(5697,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times20$}}}%
      \put(5789,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times24$}}}%
      \put(5882,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times28$}}}%
      \put(5974,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times32$}}}%
      \put(6066,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times4$}}}%
      \put(6158,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times8$}}}%
      \put(6250,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times12$}}}%
      \put(6342,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times16$}}}%
      \put(6434,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times20$}}}%
      \put(6527,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times24$}}}%
      \put(6619,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times28$}}}%
      \put(6711,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times32$}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(209,2821){\rotatebox{-270}{\makebox(0,0){\strut{}GFLOPS}}}%
      \put(3808,154){\makebox(0,0){\strut{}Micro-kernel dimensions ($m_r \times n_r$)}}%
      \csname LTb\endcsname%%
      \put(1678,4456){\makebox(0,0)[l]{\strut{}TVM}}%
      \csname LTb\endcsname%%
      \put(3061,4456){\makebox(0,0)[l]{\strut{}BLIS}}%
      \csname LTb\endcsname%%
      \put(4444,4456){\makebox(0,0)[l]{\strut{}OpenBLAS}}%
      \csname LTb\endcsname%%
      \put(5827,4456){\makebox(0,0)[l]{\strut{}ARMPL}}%
      \csname LTb\endcsname%%
      \put(3808,4709){\makebox(0,0){\strut{}Performance of GEMM on ARM Carmel - $m=401408$, $n=k=64$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={360.00bp},height={252.00bp}]{Algorithm_ARM_006-lines}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/Results/ARM/Algorithm_ARM_044-lines.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(682,1263){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(682,1782){\makebox(0,0)[r]{\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(682,2302){\makebox(0,0)[r]{\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(682,2821){\makebox(0,0)[r]{\strut{}$15$}}%
      \csname LTb\endcsname%%
      \put(682,3340){\makebox(0,0)[r]{\strut{}$20$}}%
      \csname LTb\endcsname%%
      \put(682,3860){\makebox(0,0)[r]{\strut{}$25$}}%
      \csname LTb\endcsname%%
      \put(682,4379){\makebox(0,0)[r]{\strut{}$30$}}%
      \put(906,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times4$}}}%
      \put(998,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times8$}}}%
      \put(1090,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times12$}}}%
      \put(1183,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times16$}}}%
      \put(1275,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times20$}}}%
      \put(1367,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times24$}}}%
      \put(1459,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times28$}}}%
      \put(1551,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times32$}}}%
      \put(1643,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times4$}}}%
      \put(1735,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times8$}}}%
      \put(1828,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times12$}}}%
      \put(1920,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times16$}}}%
      \put(2012,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times20$}}}%
      \put(2104,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times24$}}}%
      \put(2196,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times28$}}}%
      \put(2288,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times32$}}}%
      \put(2380,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times4$}}}%
      \put(2472,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times8$}}}%
      \put(2565,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times12$}}}%
      \put(2657,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times16$}}}%
      \put(2749,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times20$}}}%
      \put(2841,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times24$}}}%
      \put(2933,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times28$}}}%
      \put(3025,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times32$}}}%
      \put(3117,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times4$}}}%
      \put(3210,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times8$}}}%
      \put(3302,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times12$}}}%
      \put(3394,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times16$}}}%
      \put(3486,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times20$}}}%
      \put(3578,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times24$}}}%
      \put(3670,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times28$}}}%
      \put(3762,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times32$}}}%
      \put(3855,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times4$}}}%
      \put(3947,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times8$}}}%
      \put(4039,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times12$}}}%
      \put(4131,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times16$}}}%
      \put(4223,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times20$}}}%
      \put(4315,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times24$}}}%
      \put(4407,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times28$}}}%
      \put(4500,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times32$}}}%
      \put(4592,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times4$}}}%
      \put(4684,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times8$}}}%
      \put(4776,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times12$}}}%
      \put(4868,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times16$}}}%
      \put(4960,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times20$}}}%
      \put(5052,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times24$}}}%
      \put(5145,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times28$}}}%
      \put(5237,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times32$}}}%
      \put(5329,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times4$}}}%
      \put(5421,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times8$}}}%
      \put(5513,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times12$}}}%
      \put(5605,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times16$}}}%
      \put(5697,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times20$}}}%
      \put(5789,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times24$}}}%
      \put(5882,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times28$}}}%
      \put(5974,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times32$}}}%
      \put(6066,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times4$}}}%
      \put(6158,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times8$}}}%
      \put(6250,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times12$}}}%
      \put(6342,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times16$}}}%
      \put(6434,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times20$}}}%
      \put(6527,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times24$}}}%
      \put(6619,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times28$}}}%
      \put(6711,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times32$}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(209,2821){\rotatebox{-270}{\makebox(0,0){\strut{}GFLOPS}}}%
      \put(3808,154){\makebox(0,0){\strut{}Micro-kernel dimensions ($m_r \times n_r$)}}%
      \csname LTb\endcsname%%
      \put(1678,4456){\makebox(0,0)[l]{\strut{}TVM}}%
      \csname LTb\endcsname%%
      \put(3061,4456){\makebox(0,0)[l]{\strut{}BLIS}}%
      \csname LTb\endcsname%%
      \put(4444,4456){\makebox(0,0)[l]{\strut{}OpenBLAS}}%
      \csname LTb\endcsname%%
      \put(5827,4456){\makebox(0,0)[l]{\strut{}ARMPL}}%
      \csname LTb\endcsname%%
      \put(3808,4709){\makebox(0,0){\strut{}Performance of GEMM on ARM Carmel - $m=100352$, $n=512$, $k=128$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={360.00bp},height={252.00bp}]{Algorithm_ARM_044-lines}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/Results/ARM/Algorithm_ARM_all_layers.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(682,1344){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(682,1643){\makebox(0,0)[r]{\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(682,1943){\makebox(0,0)[r]{\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(682,2242){\makebox(0,0)[r]{\strut{}$15$}}%
      \csname LTb\endcsname%%
      \put(682,2542){\makebox(0,0)[r]{\strut{}$20$}}%
      \csname LTb\endcsname%%
      \put(682,2841){\makebox(0,0)[r]{\strut{}$25$}}%
      \csname LTb\endcsname%%
      \put(682,3140){\makebox(0,0)[r]{\strut{}$30$}}%
      \csname LTb\endcsname%%
      \put(682,3440){\makebox(0,0)[r]{\strut{}$35$}}%
      \csname LTb\endcsname%%
      \put(682,3739){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(1099,1124){\makebox(0,0)[r]{\strut{}1}}%
      \put(1384,1124){\makebox(0,0)[r]{\strut{}2}}%
      \put(1670,1124){\makebox(0,0)[r]{\strut{}3}}%
      \put(1955,1124){\makebox(0,0)[r]{\strut{}4}}%
      \put(2240,1124){\makebox(0,0)[r]{\strut{}5}}%
      \put(2525,1124){\makebox(0,0)[r]{\strut{}6}}%
      \put(2810,1124){\makebox(0,0)[r]{\strut{}7}}%
      \put(3096,1124){\makebox(0,0)[r]{\strut{}8}}%
      \put(3381,1124){\makebox(0,0)[r]{\strut{}9}}%
      \put(3666,1124){\makebox(0,0)[r]{\strut{}10}}%
      \put(3951,1124){\makebox(0,0)[r]{\strut{}11}}%
      \put(4236,1124){\makebox(0,0)[r]{\strut{}12}}%
      \put(4521,1124){\makebox(0,0)[r]{\strut{}13}}%
      \put(4807,1124){\makebox(0,0)[r]{\strut{}14}}%
      \put(5092,1124){\makebox(0,0)[r]{\strut{}15}}%
      \put(5377,1124){\makebox(0,0)[r]{\strut{}16}}%
      \put(5662,1124){\makebox(0,0)[r]{\strut{}17}}%
      \put(5947,1124){\makebox(0,0)[r]{\strut{}18}}%
      \put(6233,1124){\makebox(0,0)[r]{\strut{}19}}%
      \put(6518,1124){\makebox(0,0)[r]{\strut{}20}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(209,2541){\rotatebox{-270}{\makebox(0,0){\strut{}GFLOPS}}}%
      \put(3808,794){\makebox(0,0){\strut{}Layer id.}}%
      \csname LTb\endcsname%%
      \put(1577,3569){\makebox(0,0)[l]{\strut{}TVM}}%
      \csname LTb\endcsname%%
      \put(2960,3569){\makebox(0,0)[l]{\strut{}BLIS}}%
      \csname LTb\endcsname%%
      \put(4343,3569){\makebox(0,0)[l]{\strut{}OpenBLAS}}%
      \csname LTb\endcsname%%
      \put(5726,3569){\makebox(0,0)[l]{\strut{}ARMPL}}%
      \csname LTb\endcsname%%
      \put(3808,4069){\makebox(0,0){\strut{}Performance of GEMM on ARM Carmel - ResNet-50 v1.5}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={360.00bp},height={252.00bp}]{Algorithm_ARM_all_layers.eps}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/Results/ARM/Algorithm_ARM_cuadrado_2000-lines.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(682,1263){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(682,1782){\makebox(0,0)[r]{\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(682,2302){\makebox(0,0)[r]{\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(682,2821){\makebox(0,0)[r]{\strut{}$15$}}%
      \csname LTb\endcsname%%
      \put(682,3340){\makebox(0,0)[r]{\strut{}$20$}}%
      \csname LTb\endcsname%%
      \put(682,3860){\makebox(0,0)[r]{\strut{}$25$}}%
      \csname LTb\endcsname%%
      \put(682,4379){\makebox(0,0)[r]{\strut{}$30$}}%
      \put(906,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times4$}}}%
      \put(998,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times8$}}}%
      \put(1090,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times12$}}}%
      \put(1183,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times16$}}}%
      \put(1275,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times20$}}}%
      \put(1367,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times24$}}}%
      \put(1459,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times28$}}}%
      \put(1551,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times32$}}}%
      \put(1643,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times4$}}}%
      \put(1735,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times8$}}}%
      \put(1828,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times12$}}}%
      \put(1920,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times16$}}}%
      \put(2012,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times20$}}}%
      \put(2104,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times24$}}}%
      \put(2196,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times28$}}}%
      \put(2288,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times32$}}}%
      \put(2380,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times4$}}}%
      \put(2472,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times8$}}}%
      \put(2565,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times12$}}}%
      \put(2657,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times16$}}}%
      \put(2749,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times20$}}}%
      \put(2841,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times24$}}}%
      \put(2933,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times28$}}}%
      \put(3025,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times32$}}}%
      \put(3117,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times4$}}}%
      \put(3210,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times8$}}}%
      \put(3302,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times12$}}}%
      \put(3394,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times16$}}}%
      \put(3486,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times20$}}}%
      \put(3578,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times24$}}}%
      \put(3670,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times28$}}}%
      \put(3762,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times32$}}}%
      \put(3855,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times4$}}}%
      \put(3947,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times8$}}}%
      \put(4039,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times12$}}}%
      \put(4131,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times16$}}}%
      \put(4223,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times20$}}}%
      \put(4315,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times24$}}}%
      \put(4407,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times28$}}}%
      \put(4500,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times32$}}}%
      \put(4592,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times4$}}}%
      \put(4684,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times8$}}}%
      \put(4776,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times12$}}}%
      \put(4868,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times16$}}}%
      \put(4960,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times20$}}}%
      \put(5052,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times24$}}}%
      \put(5145,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times28$}}}%
      \put(5237,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times32$}}}%
      \put(5329,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times4$}}}%
      \put(5421,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times8$}}}%
      \put(5513,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times12$}}}%
      \put(5605,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times16$}}}%
      \put(5697,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times20$}}}%
      \put(5789,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times24$}}}%
      \put(5882,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times28$}}}%
      \put(5974,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times32$}}}%
      \put(6066,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times4$}}}%
      \put(6158,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times8$}}}%
      \put(6250,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times12$}}}%
      \put(6342,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times16$}}}%
      \put(6434,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times20$}}}%
      \put(6527,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times24$}}}%
      \put(6619,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times28$}}}%
      \put(6711,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times32$}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(209,2821){\rotatebox{-270}{\makebox(0,0){\strut{}GFLOPS}}}%
      \put(3808,154){\makebox(0,0){\strut{}Micro-kernel dimensions ($m_r \times n_r$)}}%
      \csname LTb\endcsname%%
      \put(1678,4456){\makebox(0,0)[l]{\strut{}TVM}}%
      \csname LTb\endcsname%%
      \put(3061,4456){\makebox(0,0)[l]{\strut{}BLIS}}%
      \csname LTb\endcsname%%
      \put(4444,4456){\makebox(0,0)[l]{\strut{}OpenBLAS}}%
      \csname LTb\endcsname%%
      \put(5827,4456){\makebox(0,0)[l]{\strut{}ARMPL}}%
      \csname LTb\endcsname%%
      \put(3808,4709){\makebox(0,0){\strut{}Performance of GEMM on ARM Carmel - $m=n=k=2000$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={360.00bp},height={252.00bp}]{Algorithm_ARM_cuadrado_2000-lines}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/Results/ARM/Algorithm_ARM_cuadrado_2000-prefetch.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(682,1263){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(682,1782){\makebox(0,0)[r]{\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(682,2302){\makebox(0,0)[r]{\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(682,2821){\makebox(0,0)[r]{\strut{}$15$}}%
      \csname LTb\endcsname%%
      \put(682,3340){\makebox(0,0)[r]{\strut{}$20$}}%
      \csname LTb\endcsname%%
      \put(682,3860){\makebox(0,0)[r]{\strut{}$25$}}%
      \csname LTb\endcsname%%
      \put(682,4379){\makebox(0,0)[r]{\strut{}$30$}}%
      \put(906,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times4$}}}%
      \put(998,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times8$}}}%
      \put(1090,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times12$}}}%
      \put(1183,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times16$}}}%
      \put(1275,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times20$}}}%
      \put(1367,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times24$}}}%
      \put(1459,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times28$}}}%
      \put(1551,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$4\times32$}}}%
      \put(1643,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times4$}}}%
      \put(1735,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times8$}}}%
      \put(1828,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times12$}}}%
      \put(1920,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times16$}}}%
      \put(2012,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times20$}}}%
      \put(2104,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times24$}}}%
      \put(2196,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times28$}}}%
      \put(2288,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$8\times32$}}}%
      \put(2380,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times4$}}}%
      \put(2472,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times8$}}}%
      \put(2565,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times12$}}}%
      \put(2657,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times16$}}}%
      \put(2749,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times20$}}}%
      \put(2841,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times24$}}}%
      \put(2933,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times28$}}}%
      \put(3025,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$12\times32$}}}%
      \put(3117,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times4$}}}%
      \put(3210,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times8$}}}%
      \put(3302,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times12$}}}%
      \put(3394,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times16$}}}%
      \put(3486,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times20$}}}%
      \put(3578,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times24$}}}%
      \put(3670,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times28$}}}%
      \put(3762,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$16\times32$}}}%
      \put(3855,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times4$}}}%
      \put(3947,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times8$}}}%
      \put(4039,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times12$}}}%
      \put(4131,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times16$}}}%
      \put(4223,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times20$}}}%
      \put(4315,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times24$}}}%
      \put(4407,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times28$}}}%
      \put(4500,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$20\times32$}}}%
      \put(4592,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times4$}}}%
      \put(4684,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times8$}}}%
      \put(4776,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times12$}}}%
      \put(4868,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times16$}}}%
      \put(4960,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times20$}}}%
      \put(5052,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times24$}}}%
      \put(5145,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times28$}}}%
      \put(5237,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$24\times32$}}}%
      \put(5329,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times4$}}}%
      \put(5421,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times8$}}}%
      \put(5513,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times12$}}}%
      \put(5605,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times16$}}}%
      \put(5697,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times20$}}}%
      \put(5789,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times24$}}}%
      \put(5882,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times28$}}}%
      \put(5974,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$28\times32$}}}%
      \put(6066,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times4$}}}%
      \put(6158,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times8$}}}%
      \put(6250,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times12$}}}%
      \put(6342,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times16$}}}%
      \put(6434,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times20$}}}%
      \put(6527,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times24$}}}%
      \put(6619,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times28$}}}%
      \put(6711,1131){\rotatebox{80}{\makebox(0,0)[r]{\strut{}\tiny$32\times32$}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(209,2821){\rotatebox{-270}{\makebox(0,0){\strut{}GFLOPS}}}%
      \put(3808,154){\makebox(0,0){\strut{}Micro-kernel dimensions ($m_r \times n_r$)}}%
      \csname LTb\endcsname%%
      \put(1678,4456){\makebox(0,0)[l]{\strut{}TVM}}%
      \csname LTb\endcsname%%
      \put(3061,4456){\makebox(0,0)[l]{\strut{}BLIS}}%
      \csname LTb\endcsname%%
      \put(4444,4456){\makebox(0,0)[l]{\strut{}OpenBLAS}}%
      \csname LTb\endcsname%%
      \put(5827,4456){\makebox(0,0)[l]{\strut{}ARMPL}}%
      \csname LTb\endcsname%%
      \put(3808,4709){\makebox(0,0){\strut{}Performance of GEMM on ARM Carmel - $m=n=k=2000$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={360.00bp},height={252.00bp}]{Algorithm_ARM_cuadrado_2000-prefetch}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/Results/Intel/Algorithm_Intel_006.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(682,1133){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(682,1782){\makebox(0,0)[r]{\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(682,2431){\makebox(0,0)[r]{\strut{}$20$}}%
      \csname LTb\endcsname%%
      \put(682,3081){\makebox(0,0)[r]{\strut{}$30$}}%
      \csname LTb\endcsname%%
      \put(682,3730){\makebox(0,0)[r]{\strut{}$40$}}%
      \csname LTb\endcsname%%
      \put(682,4379){\makebox(0,0)[r]{\strut{}$50$}}%
      \put(1054,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x4}}}%
      \put(1293,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x8}}}%
      \put(1533,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x12}}}%
      \put(1772,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x16}}}%
      \put(2012,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x32}}}%
      \put(2251,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x48}}}%
      \put(2491,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x64}}}%
      \put(2730,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x80}}}%
      \put(2970,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x96}}}%
      \put(3210,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x112}}}%
      \put(3449,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x128}}}%
      \put(3689,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x4}}}%
      \put(3928,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x8}}}%
      \put(4168,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x12}}}%
      \put(4407,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x16}}}%
      \put(4647,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x32}}}%
      \put(4887,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x48}}}%
      \put(5126,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x64}}}%
      \put(5366,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x80}}}%
      \put(5605,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x96}}}%
      \put(5845,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x112}}}%
      \put(6084,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x128}}}%
      \put(6324,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}12x16}}}%
      \put(6563,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}12x32}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(209,2756){\rotatebox{-270}{\makebox(0,0){\strut{}GFLOPS}}}%
      \put(3808,154){\makebox(0,0){\strut{}Micro-kernel dimensions ($m_r \times n_r$)}}%
      \csname LTb\endcsname%%
      \put(6011,4206){\makebox(0,0)[l]{\strut{}TVM}}%
      \csname LTb\endcsname%%
      \put(3808,4709){\makebox(0,0){\strut{}Performance of GEMM on Intel Skylake - $m=401408$, $n=k=64$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={360.00bp},height={252.00bp}]{Algorithm_Intel_006}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/Results/Intel/Algorithm_Intel_044.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(682,1133){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(682,1674){\makebox(0,0)[r]{\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(682,2215){\makebox(0,0)[r]{\strut{}$20$}}%
      \csname LTb\endcsname%%
      \put(682,2756){\makebox(0,0)[r]{\strut{}$30$}}%
      \csname LTb\endcsname%%
      \put(682,3297){\makebox(0,0)[r]{\strut{}$40$}}%
      \csname LTb\endcsname%%
      \put(682,3838){\makebox(0,0)[r]{\strut{}$50$}}%
      \csname LTb\endcsname%%
      \put(682,4379){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(1044,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x4}}}%
      \put(1275,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x8}}}%
      \put(1505,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x12}}}%
      \put(1735,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x16}}}%
      \put(1966,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x32}}}%
      \put(2196,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x48}}}%
      \put(2426,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x64}}}%
      \put(2657,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x80}}}%
      \put(2887,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x96}}}%
      \put(3117,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x112}}}%
      \put(3348,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x128}}}%
      \put(3578,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x4}}}%
      \put(3809,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x8}}}%
      \put(4039,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x12}}}%
      \put(4269,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x16}}}%
      \put(4500,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x32}}}%
      \put(4730,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x48}}}%
      \put(4960,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x64}}}%
      \put(5191,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x80}}}%
      \put(5421,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x96}}}%
      \put(5651,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x112}}}%
      \put(5882,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x128}}}%
      \put(6112,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}12x16}}}%
      \put(6342,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}32x16}}}%
      \put(6573,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}32x32}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(209,2756){\rotatebox{-270}{\makebox(0,0){\strut{}GFLOPS}}}%
      \put(3808,154){\makebox(0,0){\strut{}Micro-kernel dimensions ($m_r \times n_r$)}}%
      \csname LTb\endcsname%%
      \put(6011,4206){\makebox(0,0)[l]{\strut{}TVM}}%
      \csname LTb\endcsname%%
      \put(3808,4709){\makebox(0,0){\strut{}Performance of GEMM on Intel Skylake - $m=100352$, $n=512$, $k=128$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={360.00bp},height={252.00bp}]{Algorithm_Intel_044}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/Results/Intel/Algorithm_Intel_all_layers.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,1044){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(814,1711){\makebox(0,0)[r]{\strut{}$20$}}%
      \csname LTb\endcsname%%
      \put(814,2378){\makebox(0,0)[r]{\strut{}$40$}}%
      \csname LTb\endcsname%%
      \put(814,3045){\makebox(0,0)[r]{\strut{}$60$}}%
      \csname LTb\endcsname%%
      \put(814,3712){\makebox(0,0)[r]{\strut{}$80$}}%
      \csname LTb\endcsname%%
      \put(814,4379){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(1225,912){\rotatebox{45}{\makebox(0,0)[r]{\strut{}B3A2C0}}}%
      \put(1504,912){\rotatebox{45}{\makebox(0,0)[r]{\strut{}B3A2C0}}}%
      \put(1783,912){\rotatebox{45}{\makebox(0,0)[r]{\strut{}B3A2C0}}}%
      \put(2062,912){\rotatebox{45}{\makebox(0,0)[r]{\strut{}B3A2C0}}}%
      \put(2341,912){\rotatebox{45}{\makebox(0,0)[r]{\strut{}B3A2C0}}}%
      \put(2619,912){\rotatebox{45}{\makebox(0,0)[r]{\strut{}B3A2C0}}}%
      \put(2898,912){\rotatebox{45}{\makebox(0,0)[r]{\strut{}B3A2C0}}}%
      \put(3177,912){\rotatebox{45}{\makebox(0,0)[r]{\strut{}B3A2C0}}}%
      \put(3456,912){\rotatebox{45}{\makebox(0,0)[r]{\strut{}B3A2C0}}}%
      \put(3735,912){\rotatebox{45}{\makebox(0,0)[r]{\strut{}B3A2C0}}}%
      \put(4014,912){\rotatebox{45}{\makebox(0,0)[r]{\strut{}B3A2C0}}}%
      \put(4293,912){\rotatebox{45}{\makebox(0,0)[r]{\strut{}B3A2C0}}}%
      \put(4572,912){\rotatebox{45}{\makebox(0,0)[r]{\strut{}B3A2C0}}}%
      \put(4851,912){\rotatebox{45}{\makebox(0,0)[r]{\strut{}B3A2C0}}}%
      \put(5130,912){\rotatebox{45}{\makebox(0,0)[r]{\strut{}B3A2C0}}}%
      \put(5408,912){\rotatebox{45}{\makebox(0,0)[r]{\strut{}B3A2C0}}}%
      \put(5687,912){\rotatebox{45}{\makebox(0,0)[r]{\strut{}B3A2C0}}}%
      \put(5966,912){\rotatebox{45}{\makebox(0,0)[r]{\strut{}B3A2C0}}}%
      \put(6245,912){\rotatebox{45}{\makebox(0,0)[r]{\strut{}B3A2C0}}}%
      \put(6524,912){\rotatebox{45}{\makebox(0,0)[r]{\strut{}B3A2C0}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(209,2711){\rotatebox{-270}{\makebox(0,0){\strut{}GFLOPS}}}%
      \put(3874,154){\makebox(0,0){\strut{}Layer id.}}%
      \csname LTb\endcsname%%
      \put(1933,4206){\makebox(0,0)[l]{\strut{}TVM}}%
      \csname LTb\endcsname%%
      \put(1933,3986){\makebox(0,0)[l]{\strut{}BLIS}}%
      \csname LTb\endcsname%%
      \put(3874,4709){\makebox(0,0){\strut{}Performance of GEMM on Intel Skylake - ResNet-50 v1.5}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={360.00bp},height={252.00bp}]{Algorithm_Intel_all_layers}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/Results/Intel/Algorithm_Intel_cuadrado_2000.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(814,1133){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(814,1782){\makebox(0,0)[r]{\strut{}$20$}}%
      \csname LTb\endcsname%%
      \put(814,2431){\makebox(0,0)[r]{\strut{}$40$}}%
      \csname LTb\endcsname%%
      \put(814,3081){\makebox(0,0)[r]{\strut{}$60$}}%
      \csname LTb\endcsname%%
      \put(814,3730){\makebox(0,0)[r]{\strut{}$80$}}%
      \csname LTb\endcsname%%
      \put(814,4379){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(1089,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x4}}}%
      \put(1232,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x8}}}%
      \put(1375,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x12}}}%
      \put(1517,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x16}}}%
      \put(1660,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x20}}}%
      \put(1803,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x24}}}%
      \put(1946,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x28}}}%
      \put(2089,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x32}}}%
      \put(2232,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x36}}}%
      \put(2375,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x40}}}%
      \put(2517,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x44}}}%
      \put(2660,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x48}}}%
      \put(2803,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x52}}}%
      \put(2946,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x56}}}%
      \put(3089,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x60}}}%
      \put(3232,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x64}}}%
      \put(3375,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x80}}}%
      \put(3517,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x96}}}%
      \put(3660,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x112}}}%
      \put(3803,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}4x128}}}%
      \put(3946,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x4}}}%
      \put(4089,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x8}}}%
      \put(4232,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x12}}}%
      \put(4374,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x16}}}%
      \put(4517,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x20}}}%
      \put(4660,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x24}}}%
      \put(4803,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x28}}}%
      \put(4946,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x32}}}%
      \put(5089,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x36}}}%
      \put(5232,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x40}}}%
      \put(5374,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x44}}}%
      \put(5517,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x48}}}%
      \put(5660,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x52}}}%
      \put(5803,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x56}}}%
      \put(5946,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x60}}}%
      \put(6089,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x64}}}%
      \put(6232,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x80}}}%
      \put(6374,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x96}}}%
      \put(6517,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x112}}}%
      \put(6660,1001){\rotatebox{80}{\makebox(0,0)[r]{\strut{}8x128}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(209,2756){\rotatebox{-270}{\makebox(0,0){\strut{}GFLOPS}}}%
      \put(3874,154){\makebox(0,0){\strut{}Micro-kernel dimensions ($m_r \times n_r$)}}%
      \csname LTb\endcsname%%
      \put(6011,4206){\makebox(0,0)[l]{\strut{}TVM}}%
      \csname LTb\endcsname%%
      \put(6011,3986){\makebox(0,0)[l]{\strut{}BLIS}}%
      \csname LTb\endcsname%%
      \put(3874,4709){\makebox(0,0){\strut{}Performance of GEMM on Intel Skylake - $m=n=k=2000$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={360.00bp},height={252.00bp}]{Algorithm_Intel_cuadrado_2000}}%
    \gplfronttext
  \end{picture}%
\endgroup

